Mathematical foundation of Information Field Dynamics (revised version)

Information Field Dynamics (IFD) by Torsten En{\ss}lin provides a tool to construct simulation schemes for data vectors $d(T)$ from measurements $d(0)$ which describe certain features of a physical process (signal), without any concrete assumptions about the subgrid structure of the problem. In this work, the measure theoretical fundament and the necessary probabilistic framework for IFD are introduced first. The notation for the rest of the work is established and essential properties are developed. Afterwards, the general setting for IFD is described, consisting of the signal with its evolution equation and its linear connection to the data by a response operator. The developed environment is then used, to step by step imbed the physical language, used in Torsten En{\ss}lin's work, into a mathematical framework. Also a general approach for the approximation of an evolution equation is given, serving as a base to describe the construction of a simulation scheme with IFD. Simulation errors in the various steps are pointed out, to give an idea where inaccuracies come in and which steps therefore lead to the necessity of many degrees of freedom of the signal and of many time steps within the simulation. In the end, IFD is illustrated in an example scenario. A matrix relation for the update steps of IFD is derived. It allows to simulate a data vector $d(T)$ which averages a Klein-Gordon field with one dimension in space and periodic over $[0,2\pi)$. Also a non-iterative equation for the direct computation of $d(T)$ from $d(0)$ is constructed. This is reached by the fact that the original problem converts into an ordinary differential equation for the data, if the simulation time steps get infinitesimally small.

==> introduction/introduction_alt.tex <==
Many physical processes evoke the wish in us to predict several features of them at a prospective time, imprinted in a data vector. They are described by the state of a system, which we call the signal of interest
The underlying evolution equation of the process is very often not analytically solvable. Due to the overwhelming amount of information in the mostly infinite dimensional signal, the measured data vector for the present time contains only a limited amount of information about the process, so that one does not even know the state of the system initially. These two facts, together with the possibilities given by a computer technology, which was highly developed over the past decades, brought about the idea to simulate the physical process numerically until the time of interest, starting with the measured signal at present.
Despite the access to computer storage already expanded a lot, it is still finite though, leading to the necessity of a discretized signal within this simultion. This is why for general numerical simulations, one needs to make the implicit assumption about some subgrid structure of the evolution equation, which models the process of interest, allowing for a sufficiently close approximation of the signal by a time discrete and finite dimensional field.
By the stability of many physical processes in time, as well as by the mostly determining effect of a finite dimensional approximation of the signal on the parameters of interest, such a subgrid structure is present in many cases.
Now, analogous to the reconstruction from measurands, the idea of field reconstruction from a data vector at present time in computer memory came up. Most of such algorithms make explicit assumptions about the subgrid structure of the signal.\\
Information Field Dynamics (IFD), as introduced in \cite{enss}, provides a tool to construct simulation schemes for various physical processes, without any concrete assumptions about the subgrid structure of the problem. By measured data and assumptions on the prior statics of the underlying field, it first constructs the probability distribution of all possible field configurations of the physical process, which might have resulted in the measured data vector at present. This distribution is evolved to a later time according to the differential operator that describes the signal field dynamics. The simulated data vector is then constructed by its relation to the posterior distribution of the field at the later time, using entropic matching between this distribution and the evolved posterior. This way, a concrete connection between the measured data at present and the simulated data is developed. In this work, the necessary measure theoretical background on probability theory is introduced, and then step by step applied for the mathematical foundation of IFD. Also a general approach for the approximation of an evolution equation is given, serving as a base to describe the construction of a simulation scheme with IFD. Simulation errors in the various steps are pointed out, to give an idea where inaccuracies might come in and which steps might therefore lead to the necessity of possibly high dimensions of the discretised signal and many time steps within the simulation. In chapter \ref{chap:Maximum_Entropy_Principle}, an interpretation of relative entropy as a measure of information is given and the idea of entropic matching is explained. Chapter \ref{chap:Example: Klein-Gordon field} closes the work with an example scenario, in which a matrix is derived that allows to simulate a data vector, which averages a Klein-Gordon field in one dimension in space. In the end, also a non-iterative simulation equation is constructed for this example, using the fact that the original problem converts into an ordinary differential equation, if the simulation time steps get infinitesimally small.\\
The following picture by Torsten En\ss lin illustrates the idea of IFD.
\begin{figure}[ht]
	\centering
  \includegraphics[scale=1]{introduction/IFD9.png} 
	\label{fig1}
\end{figure}


